Post-Hoc Robustness Enhancement in Graph Neural Networks with Conditional Random Fields

Graph Neural Networks (GNNs), which are nowadays the benchmark approach in graph representation learning, have been shown to be vulnerable to adversarial attacks, raising concerns about their real-world applicability. While existing defense techniques primarily concentrate on the training phase of GNNs, involving adjustments to message passing architectures or pre-processing methods, there is a noticeable gap in methods focusing on increasing robustness during inference. In this context, this study introduces RobustCRF, a post-hoc approach aiming to enhance the robustness of GNNs at the inference stage. Our proposed method, founded on statistical relational learning using a Conditional Random Field, is model-agnostic and does not require prior knowledge about the underlying model architecture. We validate the efficacy of this approach across various models, leveraging benchmark node classification datasets.

==> chapters/limitations.tex <==
% One of the limitations of our methodology lies in its inference time. Unlike some alternative methods that may integrate robustness mechanisms directly into the training process, RobustCRF is a post-hoc method. Thus, the robustness enhancement of RobustCRF comes at a computational cost during inference. Specifically, RobustCRF necessitates multiple iterations of GNN inference. Each iteration refines the node labels based on the CRF framework, which iteratively adjusts the node predictions. As a future work, we will focus on optimizing RobustCRF to reduce its computational inference time so it can be applied in real-world scenarios where inference time is critical. 

While the proposed method is innovative, its added complexity may be seen as a limitation in certain settings (specially those related to online learning). Unlike other benchmarks in the literature that operate during the training process, RobustCRF is a post-hoc methodology. As a result, the robustness enhancement incurs a computational cost during inference. Specifically, RobustCRF requires multiple iterations of GNN inference to ensure good convergence, with each iteration refining the node labels based on the CRF framework, which iteratively adjusts the node predictions. As future work, we will focus on optimizing RobustCRF to reduce its computational inference time, making it more suitable for real-world scenarios where inference time is critical. 

%Additionally, while our current focus is on node classification, our approach can be easily adapted to other graph-related tasks, such as graph classification.
